Simple Diagnostics for Two-Way Fixed Effects

Difference-in-differences estimation is a widely used method of program evaluation. When treatment is implemented in different places at different times, researchers often use two-way fixed effects to control for location-specific and period-specific shocks. Such estimates can be severely biased when treatment effects change over time within treated units. I review the sources of this bias and propose several simple diagnostics for assessing its likely severity. I illustrate these tools through a case study of free primary education in Sub-Saharan Africa.

==> residreg.tex <==
Residualized treatment & 23.76 & -2.90 \\ 
  & (3.97) & (1.36)  \\  
  & [0.00] & [0.03]\\ 
Treatment group & 0.34 & -0.19 \\ 
  & (1.51) & (0.47)  \\  
  & [0.82] & [0.69]\\ 
Treatment group $\times$ residualized treatment & -7.81 & 5.25 \\ 
  & (6.07) & (1.99)  \\  
  & [0.20] & [0.01]\\ 


==> twfereg.tex <==
Free primary education & 20.43 & -0.47 \\ 
  & (9.12) & (3.08)  \\  
  & [0.04] & [0.88]\\ 

